Private Synthetic Data with Hierarchical Structure

We study the problem of differentially private synthetic data generation for hierarchical datasets in which individual data points are grouped together (e.g., people within households). In particular, to measure the similarity between the synthetic dataset and the underlying private one, we frame our objective under the problem of private query release, generating a synthetic dataset that preserves answers for some collection of queries (i.e., statistics like mean aggregate counts). However, while the application of private synthetic data to the problem of query release has been well studied, such research is restricted to non-hierarchical data domains, raising the initial question -- what queries are important when considering data of this form? Moreover, it has not yet been established how one can generate synthetic data at both the group and individual-level while capturing such statistics. In light of these challenges, we first formalize the problem of hierarchical query release, in which the goal is to release a collection of statistics for some hierarchical dataset. Specifically, we provide a general set of statistical queries that captures relationships between attributes at both the group and individual-level. Subsequently, we introduce private synthetic data algorithms for hierarchical query release and evaluate them on hierarchical datasets derived from the American Community Survey and Allegheny Family Screening Tool data. Finally, we look to the American Community Survey, whose inherent hierarchical structure gives rise to another set of domain-specific queries that we run experiments with.

==> checklist.tex <==
\newpage

\section*{Checklist}


% %%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section} %~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
% %%% END INSTRUCTIONS %%%


\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{In the conclusion.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{In the conclusion.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{We formulate our data universe (Section \ref{sec:domain}) and queries (Section \ref{sec:queries}). We also lay out assumptions about neighboring dataset and sensitivity in this new setting, which is crucial for deriving privacy guarantees.}
        \item Did you include complete proofs of all theoretical results?
    \answerYes{We include the proof to the privacy theorem (Theorem \ref{thm:privacy}) in the appendix.}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{We include code and instrcutions for reproducing all experimental results, except for AFST, which contains sensitive information (albeit anonymized) that cannot be released.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{We include all information in the Section \ref{sec:experiments} and the appendix.}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{Yes (over 5 runs)}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{We include this information in the appendix.}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{We cite \citet{ruggles2021ipums} (ACS) and \citet{vaithianathan2017developing} (AFST).}
  \item Did you mention the license of the assets?
    \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerYes{We include information about how we obtained access to the AFST data in the appendix.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}


\end{enumerate}

==> docs/limitations_impact.tex <==


\textbf{Limitations.} We consider data domains in which the group size $M$ is bounded, but there exists certain hierarchical datasets where $M$ can be unbounded, such as when grouping taxi trips by driver. Finally, we consider only one definition of neighboring datasets in which we protect privacy with respect to \textit{individual}-level data. Using taxi trip data as an example, one can imagine wanting to instead protect privacy with respect to both riders/trips (i.e., \textit{individual}-level) and drivers (i.e., \textit{group}-level). Finally, we focus only on categorical data, assuming that continuous attributes have already been discretized.

\textbf{Societal Impacts.} While protecting privacy has obvious positive impacts on society, differential privacy comes at the cost of introducing uncertainty and noise to statistics. Given that datasets like the ACS are already being used by researchers, introducing synthetic data as a replacement may require changes on how current stakeholders interact with the data. Moreover, deployment of such approaches may need to take into account a variety of metrics based on both the needs of stakeholders and other societal values outside of privacy (e.g., fairness).


% In this case, it may become computationally infeasible depending on the size of $M$. 
% One possible solution then is to instead treat parameterize $P_\textrm{\#}$ as some different (possible continuous or infinite) distribution and derive new functions $f_q$. 
% Finally, we consider only one definition of neighboring datasets in which we protect privacy with respect to \textit{individual}-level data. Using the taxi ride data again as example, one can imagine wanting to instead protect privacy with respect to each driver (i.e., at the \textit{group}-level). 
% In principle, there are many ways we can construct queries describing the composition of groups in $\gX$. For example, instead of asking whether a household has \textit{at least one} male (Table \ref{tab:query_types}, row $2$), one can instead ask if \textit{at least half} of individuals are male of whether the household is \textit{entirely} male. Consequently, there may exist cases in which one would need to expand the types of queries $q \in \gQ$ and derive new functions $f_q$. Moreover, w

==> notes/old1/model.tex <==
Let $S_q$ denote the set of dimensions in $\gX$ corresponding to the $k$ relevant attributes and target values for each $k$-way marginal query $\phi$. We now define $f^{\textrm{I}}_{q}$, $f^{\textrm{II}}_{q}$, and $f^{\textrm{III}}_{q}$ to differentiate between the functions for each query type that can be used to calculate answers using $G$ in \hgem.

\textit{Type I: individual-level marginal queries}
\begin{align*}
    f^{\textrm{I}}_{q}(\rvx) &= \sum_{j=1}^{M} \rvx_j \pp{\prod_{\substack{i \in S_{q} \\ i > M}} \rvx_i}
\end{align*}

\textit{Type II: group-level marginal queries}
\begin{align*}
    f^{\textrm{II}}_{q}(\rvx) &= \prod_{i \in S_{q}} \rvx_i
\end{align*}

\textit{Type III: group-contains marginal queries}
\begin{align*}
    f^{\textrm{III}}_{q}(\rvx) &= 1 - \sum_{j=1}^{M} \rvx_j \pp{1 - \prod_{i \in S_{q}} \rvx_i}^{j}
\end{align*}

As a reminder, Type III queries are a special case of hierarchical queries where $v=0$ and $\phi$ is a $k$-way marginal predicate function (i.e. $q = 1 - q^h_{\phi, v=0}$). In general, we can rewrite any statistical hierarchical query $q^h_{\phi, v}$ as
\begin{align*}
    f_{q^h_{\phi, v}}(\rvx) &= \sum_{j=1}^{M} \rvx_j {\binom{i}{v}} \pp{\prod_{i \in S_{q}} \rvx_i}^{v} \pp{1 - \prod_{i \in S_{q}} \rvx_i}^{j-v}
\end{align*}

\tl{Do we need to include probability notation so it's easier to understand?}

Therefore, we have that
\begin{equation}
f_{q}(\rvx) = 
\begin{cases} 
    f^{\textrm{I}}_{q}(\rvx) & q \in Q^{\textrm{I}} \\
    f^{\textrm{II}}_{q}(\rvx) & q \in Q^{\textrm{II}} \\
    f^{\textrm{III}}_{q}(\rvx) & q \in Q^{\textrm{III}}
\end{cases}
\end{equation}



Note that exactly $f^{\textrm{II}}_{q}$ exactly matches the definition of \textit{product queries} \citep[Definition 4]{liu2021iterative}, which \gem uses to derive answers to individual-level marginal queries. This is due to the fact that the output of \hgem (i.e. $G \pp{\rvz})$) represents distributions over \textit{groups} whereas the output of \gem represents that of individuals.

==> notes/old1/model_old.tex <==
\section{Modeling}

We introduce our algorithm, Hierarchical \gem (or \hgem), which models the joint distribution (over $\gX$) of group types using a collection of product distribution mixtures parametrized by neural networks. We derive our algorithm from \gem \citep{liu2021iterative}, which uses a single neural network to parametrizes distributions for non-hierarchical data. We describe our changes below:

\textit{Modeling.} Given some noise $\rvz \sim \gN(0, I)$, we use a multi-headed neural network $F$ in \hgem and let $F_c(\rvz)$, $F_G(\rvz)$, and $F_I(\rvz)$ denote the output of each head. In our model, $F_c(\rvz)$ defines a probability distribution over the possible number individual rows in a particular group. Meanwhile, $F_G(\rvz)$ and $F_I(\rvz)$ model the distributions of groups and of individual rows within in each group respectively. For our experiments, we use an MLP (with residual connections) for $F$, where $F_G$ is the concatenation of $M$ separate product distributions that we designate as $F_{I,1} \ldots F_{I,M}$.\footnote{This framework allows for flexibility in the number of network heads a user wants to use to represent the $M$ possible individuals found in each group. At one extreme, we can have single head such that $F_{I,i} = F_{I,j}$ $\forall i,j \le M$ (i.e., each individual is sampled from the same distribution). At the other extreme, we can model each individual separately by having a different head for each individual (i.e., $F_{I,i} = F_{I,j}$ $\forall i,j \le M$). In general, there exists many configurations, and in our implementation of \hgem that models \textit{intra-group-relationship} queries, for example, we instead create a seprate head for each person type in the ACS (e.g., all children are sampled from a neural network head that we denote as $F_{I, \textrm{child}}$).} Lastly, as in \gem, we have some batch size $B$ such that $\rvz \sim \gN(0, I_B)$, giving us $B$ total groups of product distributions to sample from uniformly. Combining all three heads, we have that $F(\rvz_i)$ is some $B \times (M + k_G + M k_I)$-dimensional output.
% \footnote{In contrast to \hgem, \gem uses a single neural network $F(\rvz_i)$ that parametrizes a distribution of individuals rows (i.e., the domain $\gI$ only)} 

\textit{Sampling.} To sample rows from $F(\rvz_i)$, we carry out a $2$-stage sampling procedure. First, we sample from $F_G(\rvz_i)$ a set of attributes in $\gG$ to define the group-level features and the number of individuals $m \sim F_c(\rvz_i)$ in each group. Subsequently, we sample $m$ sets of individual-level attributes $\gI$ according to the distribution $F_I(\rvz_i)$. Note that we will sample groups uniformly from the set of $B$ distributions parametrized by the output of $F$. For example, if $B=10$ and we wish to sample $500$ rows, we sample $50$ groups from each output $F_b(z_b)$.
% Note that we fix which \textit{individual}-level distribution $F_{I,j}$ corresponds to each group size. For notational purposes, we designate that the set of distributions $\cc{(F_G)_j \mid j = 1 \ldots m}$ correspond to individual rows in a group of size $m$ (i.e., the first row is sampled from $F_{I,1}(\rvz_i)$, the second from $F_{I,2}(\rvz_i)$, etc.).

\textit{Loss function.} Following the \adaptive framework \citep{liu2021iterative}, at each round $t$, \hgem is given a set of selected queries $\tilde{Q}_{1:t} = \cc{\tilde{q}_1, \ldots, \tilde{q}_t}$ and their noisy measurements $\tilde{M}_{1:t} = \cc{\tilde{m}_1, \ldots, \tilde{m}_t}$. Then for each query $q$, there exists a corresponding function $f_q:\sR^d\rightarrow \sR$ such that the answer given by our neural network $F$ for any query $q$ is $f_{q} \pp{F\pp{z_{j}}}$. Using $\ell_2$-norm, we have the loss function:
%
\begin{equation}\label{eq:hgem_loss}
    \gL^{\hgem} \pp{\tilde{Q}_{1:t}, \tilde{M}_{1:t}} = 
    \sum_{i=1}^{t} \norm{\tilde{m}_i - f_{\tilde{q}_i} \pp{F \pp{\rvz}} }_2
\end{equation}

\subsection{Derivation of query functions in \hgem \tl{Appendix?}} 

Starting with Definition \ref{def:normalized_query} and given some synthetic dataset $\hat{D}$ sampled from the distribution $P_\theta$ (parametrized by the parameters $\theta$ of our neural network $F$), we then have that
%
\begin{equation}\label{eq:norm_query_expectation}
    q_{\phi_1, \phi_2}(P_\theta) 
    = \mathbb{E}_{\hat{D} \sim P_{\theta}} \sbrack{q_{\phi_1, \phi_2}(\hat{D})}
    = \frac{\mathbb{E}_{\hat{D} \sim P_{\theta}} \sbrack{\sum_{x \in \hat{D}} \phi_1(x)}}{\mathbb{E}_{\hat{D} \sim P_{\theta}} \sbrack{\sum_{x \in \hat{D}} \phi_2(x)}}
\end{equation}

Next, we derive the general form of normalized queries for \hgem. In this case, each synthetic dataset sampled from \hgem can be written as $\hat{D} = \bigcup_{k=1}^{B} \hat{D}_k$ where each partition $D_k$ is sampled from the product distributions parametrized by the $k^{th}$ row in $F$. Therefore, given some predicate function $\phi = \mathbbm{1}\cc{x \in C}$, we can write
%
\begin{align*}
    \mathbb{E}_{D \sim P_{F}} \sbrack{\sum_{x \in D} \phi(x)}
    &= \sum_{k=1}^{B} \mathbb{E}_{D_k \sim P_{F_k}} \sbrack{\sum_{x \in D_k} \phi(x)} \\
    &= \sum_{k=1}^{B} \mathbb{E}_{D_k \sim P_{F_k}} \sbrack{\abs{D_k} \mathbb{E} \sbrack{\phi(x) \middle| D_k}} \\
    &= \sum_{k=1}^{B} \mathbb{E}_{D_k \sim P_{F_k}} \sbrack{\abs{D_k} P\pp{x \in C \middle| D_k}}
\end{align*}

For the queries we consider in Section \ref{sec:queries}, we have that $\phi_2 = 1$ (i.e., counts the total number of groups/individuals represented in each sample $D_k$). Therefore, we can rewrite Equation \ref{eq:norm_query_expectation} as
%
\begin{equation}\label{eq:norm_query_hgem}
    q_{\phi}(P_F) = \frac
    {\sum_{k=1}^{B} \mathbb{E}_{D_k \sim P_{F_k}} \sbrack{\abs{D_k} P\pp{x \in C \middle| D_k}}}
    {\sum_{k=1}^{B} \mathbb{E}_{D_k \sim P_{F_k}} \sbrack{\abs{D_k}}
    }
\end{equation}

To write \textit{individual-level} queries as Equation \ref{eq:norm_query_hgem}, we represent each sample from $F_k$ as a collection of individuals $D_K \in \gY$ (as described in Section \ref{sec:queries} such that $\phi$ is an indicator function. On the other hand for \textit{group-level} queries, we represent each sample as belonging to $\gX$, meaning that $D_k \in \gX$ represents a single group (and the individuals within that group). In this particular case, we have that $\abs{D_k} = 1$, reducing Equation \ref{eq:norm_query_hgem} to
%
\begin{equation*}
    q_{\phi}(P_F) = \frac{1}{B}
    \sum_{k=1}^{B} \mathbb{E}_{D_k \sim P_{F_k}} \sbrack{P\pp{x \in C \middle| D_k}}
\end{equation*}

Given that \hgem outputs a product distribution $F_G$ for \textit{group-level} attributes and separate distributions $F_I$ for each individual belonging to a group, we can conveniently switch between data domains $\gX$ and $\gY$ such that we can answer both query types with \hgem. As a result, \hgem can jointly optimize over both query types as long as $P\pp{x \in C \middle| D_k}$ can be written down as some function that is differentiable w.r.t. the parameters of $F$.

Referring to the query types found in Table \ref{tab:query_types}, we then have that
\begin{equation*}
    f_{q} \pp{F \pp{\rvz}} = \frac{1}{B} \sum_{k=1}^B \pp{\prod_{i \in S_G} \pp{F_{G}(\rvz_k)}_{i}} \pp{\sum_{m=1}^{M} \pp{F_{c}(\rvz_k)}_m \pp{1 - \prod_{j}^{m}{\pp{1 - \prod_{i \in S_I} \pp{F_{I, j}(\rvz_k)}_{i}}}}}
\end{equation*}
%
for \textit{group}-level hierarchical queries and
%
\begin{equation*}
\begin{gathered}
    f_{q} \pp{F \pp{\rvz}} = 
    \frac{f_{q, 1} 
    \pp{F \pp{\rvz}}}{f_{q, 2} \pp{F \pp{\rvz}}} \\
    f_{q, 1} \pp{F \pp{\rvz}} = 
    \sum_{k=1}^B \sum_{m=1}^M \pp{F_{c}(\rvz_k)}_m \pp{\sum_{j=1}^{m} \pp{\prod_{i \in S_I} \pp{F_{I, j}(\rvz_k)}_{i}}}
    \pp{\prod_{i \in S_G} \pp{F_{G}(\rvz_k)}_{i}} \\
    f_{q, 2} \pp{F \pp{\rvz}} = \sum_{k=1}^B \sum_{m=1}^M m \pp{F_{c}(\rvz_k)}_m
\end{gathered}
\end{equation*}    
%
for \textit{individual}-level hierarchical queries.




% Given any distribution $P$ and predicate function $\phi$ that evaluates to $\cc{0, 1}$ (i.e., and indicator function), we also have that
% \begin{align*}
%     \mathbb{E}_{D \sim P} \sbrack{\sum_{x \in D} \phi(x)}
%     &= \mathbb{E}_{P} \sbrack{\sum_{i=1}^{\abs{D}} \phi(x_i) \middle| D} \\
%     &= \mathbb{E}_{P} \sbrack{\mathbb{E} \sbrack{\sum_{i=1}^{\abs{D}} \phi(x_i) \middle| D} \middle| D} \\
%     &= \mathbb{E}_{P} \sbrack{\sum_{i=1}^{\abs{D}} \mathbb{E} \sbrack{\phi(x_i) \middle| D} \middle| D} \\
%     &= \mathbb{E}_{P} \sbrack{\sum_{i=1}^{\abs{D}} \mathbb{E} \sbrack{\mathbbm{1}\cc{x_i \in C} \middle| D} \middle| D} \\
%     &= \mathbb{E}_{D} \sbrack{\sum_{i=1}^{\abs{D}} P\pp{x_i \in C \middle| D} \middle| D} \\
%     &= \mathbb{E}_{D \sim P} \sbrack{\abs{D} P(x \in C | D)}
% \end{align*}

==> notes/old1/old_definitions.tex <==
%%%%%%

We introduce a statistical hierarchical query, which we define as the following
%
\begin{definition}[statistical hierarchical query] \label{def:hierarchical_query}
Given a hierarchical dataset $D^H = \cc{D_j}^{N_H}_{j=1}$, predicate function $\phi:\gX \rightarrow \cc{0,1}$, and target value $v$, a statistical hierarchical query is defined as
%
\begin{align*}
    q^h_{\phi, v}(D^H) = \sum^{N_H}_{j=1} \mathbbm{1}\cc{q^l_\phi(D_j) = v}
\end{align*}
%
\end{definition}
%
A statistical hierarchical query $q^h_{\phi, v}$ therefore counts the number of groups in a hierarchical dataset $D^H$ that have exactly $v$ rows satisfying some condition (defined by $\phi$). As with linear queries, $k$-way marginals can be used as the predicate function for hierarchical queries. For example, suppose we have some dataset of individuals grouped into families. Then the question---how many families have exactly one 20-year old male?---is a hierarchical query with a $2$-way marginal predicate function.

%%%%%%

Suppose now that we can represent some dataset $D^H$ as a collection of $N_H$ smaller datasets (or groups of rows) $D^H \in \gX$ (i.e., $D^H = \cc{D_j}^{N_H}_{j=1}$). We define $D^H$ as a \textit{hierarchical dataset}. Note that in total, the size of $D_H$ is $N = \sum^{N_H}_{j=1} |D_j|$.

We introduce \textit{\hcquery queries}, which we define as the following:
%
\begin{definition}[\hcquery query] \label{def:hierarchical_query}
Given a hierarchical dataset $D^H = \cc{D_j}^{N_H}_{j=1}$ and predicate function $\phi:\gX \rightarrow \cc{0,1}$, a \hcquery query is defined by the function
%
\begin{align*}
    q^h_{\phi}(D^H) = \sum_{D \in D_h}
    \mathbbm{1}\cc{\sum_{x \in D} \phi(x) > 0}
\end{align*}.
%
\end{definition}
%
A \hcquery query $q^h_{\phi}$ therefore counts the number of groups in a hierarchical dataset $D^H$ that have at least one row $x$ satisfying some condition (defined by $\phi$). As with linear queries, $k$-way marginals can be used as the predicate function for hierarchical queries. For example, suppose we have some dataset of individuals grouped into families. Then the question---how many families have exactly at least one 20-year old male?---is a \hcquery query with a $2$-way marginal predicate function.

%%%%%

We then minimize our loss function, $\gL^{\hgem}_{\theta}$, which we decompose into three parts (losses over $Q^{\textrm{I}}$, $Q^{\textrm{II}}$, and $Q^{\textrm{III}}$):
%
\begin{equation}\label{eq:gemloss}
    \gL^{\hgem}_{\theta}\pp{\tilde{Q}_{1:t}, \tilde{A}_{1:t}} = 
    \gL^{\textrm{I}}_{\theta}\pp{\tilde{Q}_{1:t}, \tilde{A}_{1:t}} +
    \gL^{\textrm{II}}_{\theta}\pp{\tilde{Q}_{1:t}, \tilde{A}_{1:t}} +
    \gL^{\textrm{III}}_{\theta}\pp{\tilde{Q}_{1:t}, \tilde{A}_{1:t}}
\end{equation}

As in \gem, we have some batch size $B$ and query function $f_q:\sR^d\rightarrow \sR$ such that the answer given by our neural network $G$ for any query $\tilde{q}$ is $\frac{1}{B} \sum_{j=1}^{B} f_{\tilde{q}_i} \pp{G\pp{z_{j}}}$. We use the notation $f^{\textrm{I}}_{q}$, $f^{\textrm{II}}_{q}$, and $f^{\textrm{III}}_{q}$ to  differentiate between the functions for each query type that can be used to calculate answers using $G_\theta$ in \hgem. We also let $S_q$ denote the set of dimensions in $\gX$ corresponding to the $k$ relevant attributes and target values for each $k$-way marginal query $\phi$.

\tl{Change notation to remove some redundancy - $\gL^{\textrm{I, II, III}}$}

\textit{Type I: individual-level marginal queries}
\begin{align*}
    \gL^{\textrm{I}}_{\theta}\pp{\tilde{Q}_{1:t}, \tilde{A}_{1:t}} &= \sum_{\tilde{q} \in Q^{\textrm{I}}} \norm{\tilde{a}_i - \frac{1}{B} \sum_{j=1}^{B} f^{\textrm{I}}_{\tilde{q}} \pp{G_\theta \pp{z_{j}}} }_p \\
    f^{\textrm{I}}_{\tilde{q}}(\rvx) &= \sum_{j=1}^{M} \rvx_j \pp{\prod_{\substack{i \in S_{\tilde{q}} \\ i > M}} \rvx_i}
\end{align*}
%
\tl{Also write the equations in probability notation so it's easier to understand?}

\textit{Type II: group-level marginal queries}
\begin{align*}
    \gL^{\textrm{II}}_{\theta}\pp{\tilde{Q}_{1:t}, \tilde{A}_{1:t}} &= \sum_{\tilde{q} \in Q^{\textrm{II}}} \norm{\tilde{a}_i - \frac{1}{B} \sum_{j=1}^{B} f^{\textrm{II}}_{\tilde{q}} \pp{G_\theta \pp{z_{j}}} }_p \\
    f^{\textrm{II}}_{\tilde{q}}(\rvx) &= \prod_{i \in S_{\tilde{q}}} \rvx_i
\end{align*}
%
Note that exactly $f^{\textrm{II}}_{\tilde{q}}$ exactly matches the definition of \textit{product queries} \citep[Definition 4]{liu2021iterative}, which \gem uses to derive answers to individual-level marginal queries. This is due to the fact that the output of \hgem (i.e. $G_\theta \pp{\rvz})$) represents distributions over \textit{groups} whereas the output of \gem represents that of individuals.

\textit{Type III: group-contains marginal queries}
\begin{align*}
    \gL^{\textrm{III}}_{\theta}\pp{\tilde{Q}_{1:t}, \tilde{A}_{1:t}} &= \sum_{\tilde{q} \in Q^{\textrm{III}}} \norm{\tilde{a}_i - \frac{1}{B} \sum_{j=1}^{B} f^{\textrm{III}}_{\tilde{q}} \pp{G_\theta \pp{z_{j}}} }_p \\
    f^{\textrm{III}}_{\tilde{q}}(\rvx) &= 1 - \sum_{j=1}^{M} \rvx_j \pp{1 - \prod_{i \in S_{\tilde{q}}} \rvx_i}^{j}
\end{align*}

As a reminder, Type III queries are a special case of hierarchical queries where $v=0$ and $\phi$ is a $k$-way marginal predicate function (i.e. $\tilde{q} = 1 - q^h_{\phi, v=0}$). In general, we can rewrite any statistical hierarchical query $q^h_{\phi, v}$ as
\begin{align*}
    f_{q^h_{\phi, v}}(\rvx) &= \sum_{j=1}^{M} \rvx_j {\binom{i}{v}} \pp{\prod_{i \in S_{\tilde{q}}} \rvx_i}^{v} \pp{1 - \prod_{i \in S_{\tilde{q}}} \rvx_i}^{j-v}
\end{align*}

==> notes/old1/preliminaries.tex <==
\section{Preliminaries}

In this work, we consider the problem of answering a collection of queries $Q$ about some private dataset $D$. To help formalize this problem, we first denote $\gX = \{0, 1\}^d$ be finite $d$-dimensional data domain. More specifically, we define this data universe $\gX$ with $d$ categorical attributes to be $\gX=\pp{\gX_{1} \times \ldots \times \gX_{d}}$, where each $\gX_{i}$ is the discrete domain of the $i$th attribute. In this case, any dataset with $N$ elements in this data universe can be written as $D = \cc{x_i}^N_{i=1}$ where $x_i \in \gX$. In the context of synthetic data generation for private query release, our goal then is to output some synthetic dataset $\hat{D}$ such that the error over all queries ($\max_{q \in Q} |q(\hat{D})-q(D)|$) is small.

We consider synthetic data generation algorithms that satisfy differential privacy \cite{DworkMNS06}, meaning that they employ randomized mechanisms $\gM:\gX^*\rightarrow \sR$ that are privacy-preserving when accessing the private dataset. 
%
\begin{definition}[Differential privacy \cite{DworkMNS06}]\label{def:dp}
A randomized mechanism $\gM:\gX^n \rightarrow \sR$ is $(\eps,\delta)$-differentially privacy, if for all neighboring datasets $D, D'$ (i.e., differing on a single person), and all measurable subsets $S\subseteq \sR$ we have:
%
\begin{align*}
    P\pp{\gM(D) \in S} \leq e^{\varepsilon} P\pp{\gM(D') \in S} + \delta
\end{align*}
%
\end{definition}

The $\ell_p$-sensitivity of function (i.e., query) captures the effect of changing an individual in the dataset and is used for deriving the noise required to be added for preserving differential privacy.
%
\begin{definition}[$\ell_p$-sensitivity]\label{def:sensitivity}
 The $\ell_p$-sensitivity of a function $f:\gX^*\rightarrow \sR^k$ is
 \begin{align*}
     \Delta f = \max_{\text{neighboring } D,D'} \| f(D) - f(D')\|_p
 \end{align*}
\end{definition}

\tl{Existing} Following a previous work on private query release, we first consider \textit{statistical linear queries}, which are otherwise known as counting queries (e.g., How many people in this dataset are \textit{male}?). More formally, we can define such queries in the following way:
%
\begin{definition}[statistical linear query] \label{def:linear_query}
Given a dataset $D$ and predicate function $\phi:\gX \rightarrow \cc{0,1}$, a statistical linear query is a defined as
%
\begin{align*}
    q^l_\phi(D) = \frac{1}{|D|} \sum_{x \in D} \phi(x)
\end{align*}
%
\end{definition}
%
Note that the predicate function $\phi$ therefore is an indicator function that outputs $1$ when the input $x$ satisfies some condition (e.g., is \textit{male}) and $0$ otherwise. In this work, we focus on $k$-way marginals for our predicate function, which we define as the following:
%
\begin{definition}[$k$-way marginal] \label{def:kway_marginal}
Given a subset $S\subseteq [d]$ of $k$ attributes and a target value $y\in \prod_{i\in S} \gX_i$ for each feature in $S$, a $k$-way marginal query is given by:
%
\begin{align*}
    \phi_{S,y}(x)= \prod_{i\in S} \mathbbm{1}\cc{x_i = y_i}
\end{align*}
%
where $x_{i} \in \gX_{i}$ means the $i$-th attribute of record $x \in \gX$. 
\end{definition}
%
In other words, the $k$-way marginal function defines some logical conjunction over $k$ attributes in $\gX$. We define each subset of attributes $S$ as a \textit{marginal}. Each marginal has a total of $\prod_{i=1}^{k} \left|\gX_{i}\right|$ queries, and we define a \textit{workload} as the set of all queries for each marginal $S$. 

\tl{New} Finally, suppose now that we can partition a dataset $D$ into $N'$ disjoint subsets of rows (i.e., $D = \bigcup^{N'}_{j=1} D_j$). Note that each group of rows $D' \in D$ can be viewed as a datset itself, with $N = \sum ^{N'}_{j=1} |D_j|$. Given this structure, we introduce \textit{\hcquery queries} as the following:
%
\begin{definition}[\hcquery query] \label{def:hierarchical_query}
Given some partitioned dataset $D = \bigcup^{N'}_{j=1} D_j$ and predicate function $\phi:\gX \rightarrow \cc{0,1}$, a \hcquery query is defined by the function \tl{notation inconsistent}
%
\begin{align*}
    q^h_{\phi}(D) = \frac{1}{N'} \sum_{D' \in D}
    \mathbbm{1}\cc{\sum_{x \in D} \phi(x) > 0}
\end{align*}
%
\end{definition}
%
A \hcquery query $q^h_{\phi}$ therefore counts the number of groups in a partitioned dataset $D$ that have at least one row $x$ satisfying some condition (defined by $\phi$). As with linear queries, $k$-way marginals can be used as the predicate function for \hcquery queries. For example, suppose we have some dataset of individuals grouped into families. Then the question---how many families have exactly at least one 20-year old male?---is a \hcquery query with a $2$-way marginal predicate function.

==> notes/old1/problem.tex <==
\section{Problem setup}

\tl{Consider adding diagram with an example dataset that illustrates what all this notation corresponds to in tabular form.}

In this paper, we consider data with some hierarchical structure, in which the data can first be partitioned in different groups that can then further be divided into individual rows. For example, one can form a hierarchical dataset from census data by grouping individuals into their respective households. Furthermore, we assume there exists some set of both \textit{group-level} (e.g., household income) and \textit{individual-level} (e.g., age) attributes, which we denote by $\gX^{(1)}=\pp{\gX^{(1)}_{1} \times \ldots \times \gX^{(1)}_{d_1}}$ and $\gX^{(2)}=\pp{\gX^{(2)}_{1} \times \ldots \times \gX^{(2)}_{d_2}}$ respectively

Let $D_1 = \cc{x_i \mid x_i \in \gX^{(1)}}^{N_1}_{i=1}$ be some \textit{individual-level} dataset and $D_2 = \cc{x_i \mid x_i \in \gX^{(2)}}^{N_2}_{i=1}$ \textit{group-level}.

In this paper, we consider a data domain $\gX$ whose $d$ attributes can be split into two subsets $\gX^{(1)}=\pp{\gX^{(1)}_{1} \times \ldots \times \gX^{(1)}_{d_1}}$ and $\gX^{(2)}=\pp{\gX^{(2)}_{1} \times \ldots \times \gX^{(2)}_{d_2}}$ where $d_1 + d_2 = d$. We designate $X^{(1)}$ as the set of \textit{group-level} attributes and $X^{(2)}$ as the set of \textit{individual-level} attributes. Given some hierarchical dataset $D^H \in \gX$ that is comprised of $N_H$ groups $D_j$, we say then that if an attribute $X^{(1)}_k$ is at the \textit{group-level}, then $X^{(1)}_k$ must be same across all elements $x_i \in D_j$. In the context of census data in which individuals are grouped into households, an example then of a person-level attribute could \textit{age}, which may vary across the members of the family, while an example of a group-level attribute may be the geographic \textit{location} of the household itself. 

Now, given this data universe, we present the following three classes of queries:

\textit{Type I: individual-level marginal queries.} The first query class is the $k$-way marginal query at the individual row level (e.g., how many individuals in my dataset are male?). This query has been well-studied in previous work \tl{(cite)} and does not take into account the hierarchical structure of $D^H$. We can therefore write this query as
%
\begin{align*}
    q^{\textrm{I}}_\phi(D) = \frac{1}{N} \sum_{D_j \in D^H} \sum_{x \in D_j} \phi_{S,y}(x)
\end{align*}
%
where $S \subseteq \gX^{(1)} \times \gX^{(2)}$. This query class has sensitivity $\frac{1}{N}$.

\textit{Type II: group-level marginal queries.} Given the hierarchical structure of our dataset, we can also then ask $k$-way marginal query at the group level (e.g., how many households in my dataset contain exactly three people?). We write this query as  \tl{Improve notation to avoid indicator function so that the function looks similar to Type I queries. Either change $D_j$ or add a new $\phi$ just for group-level predicate functions.}
%
\begin{align*}
    q^{\textrm{II}}_\phi(D) = \frac{1}{N_H} \sum_{D_j \in D^H} \mathbbm{1}\cc{\phi_{S,y}(D_j) = |D_j|}
\end{align*}
%
where $S \subseteq \gX^{(2)}$. This query class has sensitivity $\frac{1}{N_H}$.

\textit{Type III: \hcquery marginal queries.} Finally, our third class of queries counts the number of groups that contain at least one individual satisfying some $k$-way marginal predicate function (e.g., how many households in my dataset contain at least one person seeking employment?). We write this query as
%
\begin{align*}
    q^{\textrm{III}}_\phi(D) 
    &= \frac{1}{N_H} \sum^{N_H}_{j=1} \mathbbm{1}\cc{q^l_\phi(D_j) > 0} \\
    &= 1 - \frac{1}{N_H} \sum^{N_H}_{j=1} \mathbbm{1}\cc{q^l_\phi(D_j) = 0}
\end{align*}
%
where $S \subseteq \gX^{(1)}$. Note that this is the equivalent to the negation of a statistical hierarchical query where $v=0$. This query class has sensitivity $\frac{1}{N_H}$.

In the following section, we will use the symbols $Q^{\textrm{I}}$, $Q^{\textrm{II}}$, and $Q^{\textrm{III}}$ to denote sets containing query types I, II, III respectively (i.e., $Q = Q^{\textrm{I}} \cup Q^{\textrm{II}} \cup Q^{\textrm{III}}$).

\section{Modeling}

We assume that each group contains at most $M$ rows (i.e., $|D_j| \le M$). We also assume that the first group-level attribute $\gX^{(2)}_{1}$ always designates the number of individuals found in the group (i.e., $\sf{COUNT}$) and that $\gX^{(2)}_{1}$ corresponds to the dimensions $1 \ldots M$ in $\gX$. 

\subsection{Hierarchical MWEM/PEP}

\tl{Placeholder, but I don't think we need this, especially since it takes away from \hgem.}

\subsection{Hierarchical GEM}

\tl{Language needs to adjustments so that it doesn't seem like it's some trivial extension to \gem}. 

We introduce our algorithm, Hierarchical \gem (or \hgem), which also models the data as mixtures of product distributions using the \adaptive iterative procedure. However to capture the hierarchical structure of the private dataset and optimize over query types II and II, we make following modifications to \gem: 

\textit{Modeling.} Given some noise $\rvz \sim \gN(0, \sigma^2 I)$, the neural network $G$ in \hgem outputs two sets of product distributions, $G^{(1)}(\rvz)$ and $G^{(2)}(\rvz)$, that model the distributions of groups and of individual rows within in each group respectively. In contrast, $G(\rvz_i)$ in \gem is instead some distribution of individuals rows (i.e., the domain $\gX^{(2)}$ only). For our experiments we use a single MLP to generate both $G^{(1)}$ and $G^{(2)}$, where $G^{(2)}$ is comprised of $M$ separate product distributions that we designate as $G_1^{(2)} \ldots G_M^{(2)}$. $G(\rvz_i)$ is thus a $(d_1 + M d_2)$-dimensional vector. Finally, we fix which distributions $G_j^{(2)}$ correspond to each group size. Specifically, the set of distributions $\cc{G_j^{(2)} \mid j = 1 \ldots m}$ correspond to individual rows in a group of size $m$. 

\textit{Sampling.} To sample rows from $G(\rvz_i)$, we carry out a $2$-stage sampling procedure. First, we sample a set of attributes $\gX^{(1)}$ from $G^{(1)}(\rvz_i)$ to define the group-level features. Note that the attribute $\gX^{(2)}_{1}$ determines $m$, the number of individuals contained in this group sample. Subsequently, we then sample $m$ rows of individual-level attributes $\gX^{(1)}$ according to the distribution $G^{(1)}(\rvz_i)$ (i.e., the first row is sampled from $G_1^{(1)}(\rvz_i)$, the second from $G_2^{(1)}(\rvz_i)$, etc.)

\textit{Loss function.} Following the \adaptive framework, at each round $t$, \hgem is given a set of selected queries $\tilde{Q}_{1:t} = \cc{\tilde{q}_1, \ldots, \tilde{q}_t}$ and their noisy measurements $\tilde{A}_{1:t} = \cc{\tilde{a}_1, \ldots, \tilde{a}_t}$. As in \gem, we have some batch size $B$ and query function $f_q:\sR^d\rightarrow \sR$ such that the answer given by our neural network $G$ for any query $q$ is $\frac{1}{B} \sum_{j=1}^{B} f_{q} \pp{G\pp{z_{j}}}$. Using $\ell_p$-norm, we then have the following loss function:
%
\begin{equation}\label{eq:hgemloss}
    \gL^{\hgem} \pp{\tilde{Q}_{1:t}, \tilde{A}_{1:t}} = 
    \sum_{\tilde{q} \in \tilde{Q}} \norm{\tilde{a}_i - \frac{1}{B} \sum_{j=1}^{B} f_{\tilde{q}} \pp{G \pp{z_{j}}} }_p
\end{equation}

Let $S_q$ denote the set of dimensions in $\gX$ corresponding to the $k$ relevant attributes and target values for each $k$-way marginal query $\phi$. We now define $f^{\textrm{I}}_{q}$, $f^{\textrm{II}}_{q}$, and $f^{\textrm{III}}_{q}$ to differentiate between the functions for each query type that can be used to calculate answers using $G$ in \hgem.

\textit{Type I: individual-level marginal queries}
\begin{align*}
    f^{\textrm{I}}_{q}(\rvx) &= \sum_{j=1}^{M} \rvx_j \pp{\prod_{\substack{i \in S_{q} \\ i > M}} \rvx_i}
\end{align*}

\textit{Type II: group-level marginal queries}
\begin{align*}
    f^{\textrm{II}}_{q}(\rvx) &= \prod_{i \in S_{q}} \rvx_i
\end{align*}

\textit{Type III: group-contains marginal queries}
\begin{align*}
    f^{\textrm{III}}_{q}(\rvx) &= 1 - \sum_{j=1}^{M} \rvx_j \pp{1 - \prod_{i \in S_{q}} \rvx_i}^{j}
\end{align*}

As a reminder, Type III queries are a special case of hierarchical queries where $v=0$ and $\phi$ is a $k$-way marginal predicate function (i.e. $q = 1 - q^h_{\phi, v=0}$). In general, we can rewrite any statistical hierarchical query $q^h_{\phi, v}$ as
\begin{align*}
    f_{q^h_{\phi, v}}(\rvx) &= \sum_{j=1}^{M} \rvx_j {\binom{i}{v}} \pp{\prod_{i \in S_{q}} \rvx_i}^{v} \pp{1 - \prod_{i \in S_{q}} \rvx_i}^{j-v}
\end{align*}

\tl{Do we need to include probability notation so it's easier to understand?}

Therefore, we have that
\begin{equation}
f_{q}(\rvx) = 
\begin{cases} 
    f^{\textrm{I}}_{q}(\rvx) & q \in Q^{\textrm{I}} \\
    f^{\textrm{II}}_{q}(\rvx) & q \in Q^{\textrm{II}} \\
    f^{\textrm{III}}_{q}(\rvx) & q \in Q^{\textrm{III}}
\end{cases}
\end{equation}



Note that exactly $f^{\textrm{II}}_{q}$ exactly matches the definition of \textit{product queries} \citep[Definition 4]{liu2021iterative}, which \gem uses to derive answers to individual-level marginal queries. This is due to the fact that the output of \hgem (i.e. $G \pp{\rvz})$) represents distributions over \textit{groups} whereas the output of \gem represents that of individuals.

==> notes/old2/model.tex <==
\section{Synthetic data generation for hierarchical data}\label{sec:modeling}
 
Having formulated the problem of hierarchical query release, we next introduce a general framework for answering queries privately via synthetic data generation, in which the goal is to solve the optimization problem $\min_{\hat{D} \in \gD} \max_{q \in \gQ} | q(D) - q(\hat{D})|$ for some family of distributions $\gD$. In particular, we consider algorithms under the \adaptive framework \citep{liu2021iterative}, which we write down in Algorithm \ref{alg:adaptive} with the \textit{exponential} and \textit{Gaussian} mechanisms for the sample and measure steps. In addition, we run these two mechanisms under the assumption that all queries $q \in \gQ$ have $\ell_1$-sensitivity equal to $\max_{q \in \gQ} \Delta_1\pp{q}$ (i.e., $\frac{1}{N_G}$ for $\gQ = \gQ_G \cup \gQ_I$), allowing us to preserve the privacy guarantees presented in \citet[Theorem 1]{liu2021iterative}:

\begin{theorem}
When run with privacy parameter $\rho$, \adaptive satisfies $\rho$-zCDP. Moreover for all $\delta>0$, algorithms under the \adaptive framework satisfies $\pp{\varepsilon(\delta), \delta}$-differential privacy, where $\varepsilon(\delta) \le \rho + 2\sqrt{\rho\log(1/\delta)}$.
\label{thm:privacy}
\end{theorem}

\input{algos/adaptive}

As \citet{liu2021iterative} demonstrates, algorithms under this framework can then be reduced to selecting $\gD$ (and a corresponding loss function w.r.t. $\gD$ and $\gQ$). 

\iffalse
One simple solution is to let $\gD$ be all distributions of the support of $\gG$. From there, one can run algorithms, such as \mwem \citep{HardtLM12}, to optimize some loss function $\gL$. However, in most practical settings, such algorithms are computationally intractable, given that the memory and computational requirements these algorithms scale with the size of $\gX$. 

Inspired by methods introduced in \citet{liu2021iterative}, we then demonstrate that an alternative solution is to represent $\gD$ as a set of product distributions over each attribute in $\gI$ and $\gG$. In this way, the computational requirements for methods operating on $\gD$ scale only \textit{linearly} with respect to $M$ and the number of attributes $k_G$ and $k_I$. From there, we provide two ways in which one can parameterize $\gD$ and derive a differentiable loss function for each hierarchical query.
\fi



\subsection{Explicit distribution over the support of $\gX$}

First, we consider algorithms that optimize over the distributional family $\gD = \cc{\rvx \mid \rvx \in [0, 1]^d, \norm{\rvx}_1 = 1}$. In other words, $\gD$ contains all possible probability distributions over $\gX$, and any histogram $A \in \gD$ can be thought of as a normalized histogram over group types in $\gX$. In this case, the parameters of methods optimizing over such representations are simply the values of a $|\gX|$-dimensional probability vector. Furthermore, we can also sample directly from $A_D$ to generate a synthetic dataset $\hat{D} \in \gX$.

Suppose we have some dataset $D \in \gX$ with some group size $N_G$ and histogram representation $A_D \in \gD$. Then, we can write any \linear (Definition \ref{def:linear_query}) as a dot product $q_{\phi}(D) = N_G \langle \vec{q}_\phi, A_D \rangle$ and $\vec{q}_\phi = \lbrack \phi(\rvx_1), \ldots, \phi(\rvx_d) \rbrack$. We now discuss how to evaluate both \textit{group} and \textit{individual-level} queries on a histogram $A \in \gD$.

\textit{Group-level queries} ($\gQ_G$).
%
Given that $A$ is a distribution over all possible group types, we have that $\phi:\gX \rightarrow \cc{0, 1}$. Moreover, since we are normalizing over some total number of groups $N_G$ for \textit{group}-level queries, our query function $f_q$ for some query with predicate $\phi$ is simply
%
\begin{align*}
    f_{q}(A) = \frac{1}{N_G} q_{\phi}(A) = \langle \vec{q}_\phi, A \rangle
\end{align*}

\textit{Individual-level queries} ($\gQ_I$).
%
A group can contribute up to $M$ individuals when counting the number of individuals satisfying some predicate condition $\phi:\gX \rightarrow \cc{0, 1, \ldots, M}$. Moreover, even when $N_G$ is fixed, the number of individual rows contained in $D$ varies with $A_D$. Let $\phi_{\#}:\gX \rightarrow \cc{1, 2, \ldots, M}$ be the predicate function that outputs the size of a group $x \in \gX$. Then the total number of individual rows in $D$ is $N_I = N_G \langle \vec{q}_{\phi_{\#}}, A_D \rangle$. Therefore for \textit{individual}-level queries, we have that
%
\begin{align*}
    f_{q}(A) = \frac{1}{N_I} q_{\phi}(A) = \frac{ \langle \vec{q}_{\phi}, A \rangle}{\langle \vec{q}_{\phi_{\#}}, A \rangle}
\end{align*}

Having described how to both parameterize $\gX$ and evaluate any hierarchical query $q$ on some dataset $D \in \gX$, one can directly optimize our objective using algorithms such as the \textit{multiplicative weights} update rule (i.e., the \mwem algorithm \citep{HardtLM12}, which we describe in Appendix \ref{appx:mwem}). 

\subsection{Hierarchical product distributions (HPD)}

In the non-hierarchical setting (i.e. data only at the \textit{individual-level}), \citet{liu2021iterative} demonstrate that one can represent any data domain $\gI$ as product distributions over each attribute in $\gI$, which we denote as $P_{\gI}$. However, in the hierarchical setting, there exists attributes at the \textit{group-level}, requiring us to model a separate distribution $P_{\gG}$ over $\gG$ as well. Moreover, given that each household has at most $M$ individuals, we propose maintaining a separate distribution $P_{\gI_{i}}$ for $i \in \cc{1, 2, \ldots, M}$, where each $P_{\gI_{i}}$ corresponds to the $i^{th}$ possible person in a household. Finally, because the size of a group can vary (i.e., $\tilde{\gI}$ may be a non-existent individual row $\perp$), we let $P_{\textrm{\#}}$ be a discrete distribution over possible group sizes $m$. We let $P$ be the overall distribution over $\gX$  given by $P_{\textrm{\#}}$, $P_{\gG}$, and $P_{\gI_{i}}$ for $i \in \cc{1, 2, \ldots, M}$.

\input{algos/hpd_sampling}

\textit{Mixture of product distributions.}
%
Modeling any dataset $D$ using $P_{\textrm{\#}}$, $P_{\gG}$, and $P_{\gI_{i}}$ assumes that for all groups and the individual rows contained each group, attributes are independent. Therefore, we maintain a set of $K$ product distributions $P^{(k)}$ for $k \in \cc{1, 2, \ldots, K}$, where $K$ is some tunable parameter that increases the expressiveness of our probability distribution $P$.
For example, dataset $D$ of size $N$ can be perfectly captured by a set of $K = N$ product distributions (i.e., a product distribution of point masses for each row in $D$). Going forward, we let $P = \cc{P^{(1)}, P^{(2)}, \ldots, P^{(K)}}$. In total then, $P$ is parameterized by $K \times (M + |\gG| + M |\gI|)$ values (which is grows linearly with the number of attributes). To sample from $P$, we first sample uniformly some $P^{(k)}$ from the set of $K$ distributions and then follow the sampling procedure summarized in Algorithm \ref{alg:hpd_sampling}.

% \textit{Sampling.} 
% %
% To sample rows from $P_{\textrm{hier}}$, we propose a simple $2$-stage sampling procedure. First, we sample from $P_{\gG}$ a set of attributes in $\gG$ to define the group-level features, as well as the number of individual rows $m$ in each group from $P_{\textrm{\#}}$. Subsequently, we sample $m$ sets of individual-level attributes $\gI$ according to the distributions $P_{\gI_{1}}, P_{\gI_{2}}, \ldots, P_{\gI_{M}}$. Note that we will sample groups uniformly from each $P_{\textrm{hier}}^{(k)}$ (e.g., if $K=10$ and we wish to sample $500$ rows for our synthetic dataset, we sample $50$ groups from each distribution $P_{\textrm{hier}}^{(k)}$).
% (i.e. in a group of size $m$, $P_{\gI_{1}}, P_{\gI_{2}}, \ldots, P_{\gI_{M}}$ are designated as the distributions from which individual row's attributes are drawn from)

\subsubsection{Modeling}

We now show how one can derive iterative algorithms for hierarchical data under the \adaptive framework \citep{liu2021iterative}. In particular, having restricted our family of distributions $\gD$ over $X$ to the set of product distributions $P_{\textrm{hier}}$, we simply need to (1) parametrize $P_{\textrm{hier}}$ and (2) derive a loss function that is differentiable w.r.t to such parameters.

\textit{Parametrizing $P_{\textrm{hier}}$.} 
%
In this setting, any algorithm must output some $d_{\textrm{hier}}$-dimensional vector that is made up of the probability vectors in  $P_{\textrm{hier}}$. For notational purposes, we will let $\vect{P}^{\gG}$ be a $(K \times |\gG|)$-dimensional matrix where each row vector $\vect{P}^{\gG}_k$ corresponds to \textit{group-level} distribution $P_{\gG}^{(k)}$. Similarly, let $\vect{P}^{\gI_{i}}$ be a $(K \times |\gI|)$-dimensional matrix corresponding to $P_{\gI_{i}}$ for each $i \in \cc{1, 2, \ldots, M}$ and $\vect{P}^{\textrm{\#}}$ be a $(K \times M)$-dimensional matrix corresponding to $P_{\textrm{\#}}$.
%
% \footnote{Note that since we have a separate matrix parameterizing $\gG$, $\gI_i$ and $M$, it is simple to switch between viewing $P_\textrm{hier}$ as a distribution over either \textit{groups} ($\gG$) or \textit{individuals} ($\gI$). Similarly, calculating \normcountings at the \textit{group-level} and \textit{individual-level} is equivalent to looping over each row in $\vect{P}^{\gG}$ and $\vect{P}^{\gI_{i}}$ respectively.}

We describe two methods for parameterizing $P_{\textrm{hier}}$ that are inspired by \rapsoftmax and \gem \citep{liu2021iterative}. The first of which maintains a fixed distribution in which the parameters of our model are exactly the probabilities vectors that comprise $P_{\textrm{hier}}$, and the second of which employs generative modeling by employing some neural network architecture that takes as input randomly sampled Gaussian noise $\vect{z}$. Note that in both cases, we use the softmax function over dimensions corresponding to each attribute to output probabilty matrices $\vect{P}^{\gG}$, $\vect{P}^{\gI_{i}}$, and $\vect{P}^{\textrm{\#}}$. 

\textbf{Fixed distribution modeling (\fixed).} 
%
Our first method simply defines a "model" whose parameters $\theta^{\gG}$, $\theta^{\gI_{i}}$, and $\theta^{\textrm{\#}}$ are simply the  matrices $\vect{P}^{\gG}$, $\vect{P}^{\gI_{i}}$, and $\vect{P}^{\textrm{\#}}$ respectively.

\textbf{Generative modeling (\generative).} 
%
Alternatively, we propose using a a multi-headed neural network $F$ to generate rows from Gaussian noise $\rvz \sim \gN(0, I_{K})$. In this case, the output of each head, which we denote by $F^{\gG}(\rvz)$, $F^{\gI_{i}}(\rvz)$, and $F^{\textrm{\#}}(\rvz)$, corresponds to the $\vect{P}^{\gG}$, $\vect{P}^{\gI_{i}}$, and $\vect{P}^{\textrm{\#}}$ respectively.

% For our experiments, we use an MLP (with residual connections) for $F$, where $F_G$ is the concatenation of $M$ separate product distributions that we designate as $F_{I,1} \ldots F_{I,M}$. 

% We present two methods optimizing $P_{\textrm{hier}}$ over some set of hierarchical queries $\gQ$, the former being inspired by \rapsoftmax

\textit{Loss function.}
%
Following the \adaptive framework \citep{liu2021iterative}, at each round $t$, we have a set of selected queries $\tilde{Q}_{1:t} = \cc{\tilde{q}_1, \ldots, \tilde{q}_t}$ and their noisy measurements $\tilde{M}_{1:t} = \cc{\tilde{m}_1, \ldots, \tilde{m}_t}$. Suppose we have some set of probability matrices $\vect{P}^{\gG}$, $\vect{P}^{\gI_{i}}$ for $i \in \cc{1, 2, \ldots, M}$, and $\vect{P}^{\textrm{\#}}$ that are generated via either fixed distribution or generative modeling methods outlined above. Abusing notation, we use $\vect{P}$ to denote the collection of these matrices. Taken together, we then have that at each round $t$, we optimize the following loss function:
%
\begin{equation}\label{eq:hpd_loss}
    \gL^{\hpd} \pp{\vect{P}, \tilde{Q}_{1:t}, \tilde{M}_{1:t}} = 
    \sum_{i=1}^{t} \norm{\tilde{m}_i - f_{\tilde{q}_i} \pp{\vect{P}} }_2
\end{equation}
%
where for query $q$, there exists a corresponding function $f_q$ that maps from $\vect{P}^{\gG}$, $\vect{P}^{\gI_{i}}$ for $i \in \cc{1, 2, \ldots, M}$, and $\vect{P}^{\textrm{\#}}$ to the corresponding query answer. In particular, we have that (referring to the query types in Table \ref{tab:query_types}
%
\begin{equation*}
    f_{q} \pp{\vect{P}} = 
    \frac{1}{K} \sum_{k=1}^K \pp{\prod_{i \in S_G} \vect{P}^{\gG}_{ki}} 
    \pp{\sum_{m=1}^{M} \vect{P}^{\textrm{\#}}_{km} \pp{1 - \prod_{j=1}^{m}{\pp{1 - \prod_{i \in S_I} \vect{P}^{\gI_{j}}_{ki} }}}}
\end{equation*}
%
for \textit{group}-level hierarchical queries ($\gQ_G$) and
%    

\begin{equation*}
    \left.
    f_{q} \pp{\vect{P}} = 
    \frac{1}{K} \sum_{k=1}^K 
    \pp{\prod_{i \in S_G} \vect{P}^{\gG}_{ki}} 
    \pp{\sum_{m=1}^M \vect{P}^{\textrm{\#}}_{km} \sum_{j=1}^{m} \pp{\prod_{i \in S_I} \vect{P}^{\gI_{j}}_{ki} }}
    \middle/
    \sum_{k=1}^K 
    \pp{\sum_{m=1}^M m \vect{P}^{\textrm{\#}}_{km}}
    \right.
\end{equation*}   
%
for \textit{individual}-level hierarchical queries ($\gQ_I$).
% \begin{equation*}
% \begin{gathered}
%     f_{q} \pp{\vect{P}} = 
%     \frac{f_{q, 1} 
%     \pp{\vect{P}}}{f_{q, 2} \pp{\vect{P}}} \\
%     f_{q, 1} \pp{\vect{P}} = 
%     \sum_{k=1}^K \sum_{m=1}^M \vect{P}^{\textrm{\#}}_{km} \pp{\sum_{j=1}^{m} \pp{\prod_{i \in S_I} \vect{P}^{\gI_{j}}_{ki} }}
%     \pp{\prod_{i \in S_G} \vect{P}^{\gG}_{ki}} \\
%     f_{q, 2} \pp{\vect{P}} = \sum_{k=1}^K \sum_{m=1}^M m \vect{P}^{\textrm{\#}}_{km}
% \end{gathered}
% \end{equation*} 

==> notes/old2/preliminaries.tex <==
\section{Preliminaries}

We study the problem of answering a collection of queries $Q$ about some private dataset $D$. To formalize this problem, we first let \swedit{$\gX = \{0, 1\}^d$} denote some data domain of \swedit{dimension} $d$. As a result, any dataset can be represented as some histogram \swedit{$D \in \sN^{|\gX|}$} over elements in $\gX$.\swcomment{do we ever use this representation} In the context of synthetic data generation for private query release, our goal then is to output some synthetic dataset $\hat{D}$ such that the error over all queries ($\max_{q \in Q} |q(\hat{D})-q(D)|$) is small. 

We consider synthetic data generation algorithms that satisfy differential privacy \citep{DworkMNS06}, meaning that they employ randomized mechanisms $\gM:\gX^*\rightarrow \sR$ that are privacy-preserving when accessing the private dataset. 
%
\begin{definition}[Differential privacy \citep{DworkMNS06}]\label{def:dp}
A randomized mechanism $\gM:\gX^n \rightarrow \sR$ is $(\varepsilon,\delta)$-differentially privacy, if for all neighboring datasets $D, D'$ (i.e., differing on a single person), and all measurable subsets $S\subseteq \sR$ we have:
%
\begin{align*}
    P\pp{\gM(D) \in S} \leq e^{\varepsilon} P\pp{\gM(D') \in S} + \delta
\end{align*}
%
\end{definition}

% \footnote{In some works, \textit{statistical linear queries} are defined in the same way, with the exception that the output is normalized by the size of the dataset.}

Next, the $\ell_p$-sensitivity of a function captures the effect of changing an individual in the dataset and is used for deriving the added noise required to preserve privacy guarantees at various budgets $(\varepsilon,\delta)$.
%
\begin{definition}[$\ell_p$-sensitivity]\label{def:sensitivity}
The $\ell_p$-sensitivity of a function $f:\gX^*\rightarrow \sR^k$ is
\begin{align*}
    \Delta_p f = \max_{\text{neighboring } D,D'} \| f(D) - f(D')\|_p
\end{align*}

\end{definition}

We now introduce our definition of a \textit{\linear} as the following:
%
\begin{definition}[\linear] \label{def:linear_query}
Given a dataset $D$ and predicate function $\phi:\gX \rightarrow \sR$, a \linear is defined as
%
\begin{align*}
    q_\phi(D) = \sum_{x \in D} \phi(x)
\end{align*}
%
\end{definition}

For example, the number of males in some dataset can be represented as a \linear with a predicate function $\phi(x) = \mathbbm{1}\cc{x \textrm{ is male}}$. In the case where $\phi$ is an indicator function, the output of some \linear $q_{\phi}(D)$ can be thought of as some count of elements $x \in D$ satisfying a condition defined by $\phi$ (e.g., \textit{is male}). Going forward, we will refer to such conditions as \textit{predicate conditions}. Similar to previous work, we will normalize query answers with respect to some fixed constant $N$,
%
\footnote{In some previous works, \linear is defined with the normalizing constant included (where $N = |D|$)} 
%
such as the total number of rows in the dataset (e.g. \% \textit{males} = \# \textit{males} / \# \textit{people}). 

Finally, following previous work on private query release, we will focus our attention to tabular data with columns that are either categorical or discretized, using $k$-way marginals for our predicate $\phi$.
%
\begin{definition}[$k$-way marginal] \label{def:kway_marginal}
Given a subset $S\subseteq [d]$ of $k$ attributes and a target value $y\in \prod_{i\in S} \gX_i$ for each feature in $S$, a $k$-way marginal query is given by:
%
\begin{align*}
    \phi_{S,y}(x)= \prod_{i\in S} \mathbbm{1}\cc{x_i = y_i}
\end{align*}
%
where $x_{i} \in \gX_{i}$ means the $i$-th attribute of record $x \in \gX$. 
\end{definition}
%
In other words, $k$-way marginals define some logical conjunction over predicate conditions defined for $k$ distinct attributes in $\gX$.



\iffalse
We formally define such statistical queries as:
\swcomment{small subtlety: i think it might be easier to think of n being fixed, and neighboring means replacing a person with another}

%
\begin{definition}[\normalized] \label{def:normalized_query}
Given a dataset $D$ and predicate functions $\phi_1, \phi_2 :\gX \rightarrow \sR$, a \normalized is a defined as \swcomment{maybe call it ratio query?}
%
\begin{align*}
    q^{norm}_{\phi_1, \phi_2}(D) = \frac{q^{lin}_{\phi_1}(D)}{q^{lin}_{\phi_2}(D)}
\end{align*}
%
where for all $x \in \gX$, $\phi_1(x) \le \phi_2(x)$.
\end{definition}

Under this definition, \normalizeds can be used to define conditional statistics, such as---\textit{What fraction of males in my dataset are white?} (i.e., $\phi_1(x) = \mathbbm{1}\cc{x \textrm{ is male and white}}$ and $\phi_2(x) = \mathbbm{1}\cc{x \textrm{ is male}}$). Similarly, statistical queries that output counts as a fraction of rows in the dataset (rather than the total) can be reduced to the simple case in which $\phi_1(x)\in \cc{0, 1}$ and $\phi_2(x) = 1$ for all $x \in \gX$ (i.e., $q^{linear}_{\phi_2}(D) = |D|$ counts the total number of rows in $D$). \swcomment{first time seeing SQ} Thus, \normalizeds are linear in $D$ in this special case---which we will refer to as \textit{\normcountings}---and only need to be defined w.r.t. a single indicator function $\phi$ (i.e. $q^{norm}_{\phi}(D) = \frac{1}{|D|} q_{\phi}(D)$).
% In this paper, will refer to this special case of counting queries $ q^{norm}_{\phi}(D) = \frac{1}{|D|} q^{linear}_{\phi}(D)$ as \textit{normalized linear queries}\footnote{In contrast to this paper, previous works in the literature instead define \textit{statistical linear queries} as this special case of Definition \ref{def:normalized_query}.}.

\fi

==> notes/old2/problem.tex <==
\section{Hierarchical Counting Queries}\label{sec:queries}

We consider data with some hierarchical structure, in which the data can first be partitioned into different groups that can then further be divided into individual rows. For example, one can form a hierarchical dataset from census data by grouping individuals into their respective households. We assume that each group contains at most $M > 1$ rows and has $k_G$ features $\gG = \pp{\gG_{1} \times \ldots \times \gG_{k_G}}$. Similarly, we assume that each individual row belongs to some data domain of $k_I$ features $\gI = \pp{\gI_{1} \times \ldots \times \gI_{k_I}}$. For example, a census survey may record whether households reside in an urban or rural area ($\gG = \textsc{Urban/Rural}$) and what the sex and race ($\gI = \textsc{Sex} \times \textsc{Race}$) are of individuals in each household.\swcomment{the example you gave makes it look like $\gI$ and $\gG$ only have one attribute} Putting these attribute domains together, we then have a hierarchical data universe
%
\begin{equation*}
    \gX = \gG \times \tilde{\gI}^M,
\end{equation*}
%
where $\tilde{\gI} = \gI \times \perp$ and $\perp$ represents an empty set of features in $\gI$ (i.e., one of the $M$ possible individual rows do not exist in the group). Letting the \textit{group}-level domain size $d_G = \prod_{i=1}^{k_G} |\gG_i|$ and \textit{individual}-level domain size $d_I = \prod_{i=1}^{k_I} |\gI_i|$, the overall domain size can be written as $d = d_G \sum_{i=1}^{M} \pp{d_I}^i$. Conveniently, this formulation also allows us to convert hierarchical datasets from a collection of groups $D \in \gX$ to a collection individuals $D \in \gY$ where
%
\begin{equation*}
    \gY = \gI \times \gG \times \tilde{\gI}^{M-1}
\end{equation*}
%
with $\gI$ defining the features for some individual row $x$, $\gG$ the group to which $x$ belongs, and $\tilde{\gI}^{M-1}$ the remaining rows belonging to the same group. \tl{do we still need this?}

Having grouped the attributes of our hierarchical domain into \textit{group} and \textit{individual}-level attributes $\gG$ and $\gI$, we now introduce two classes of queries: \textbf{(1)} \linears at the \textbf{\textit{group}}-level $\gQ_G$ (e.g., \% of households) and \textbf{(2)} \linears at the \textbf{\textit{individual}}-level $\gQ_I$ (e.g. \% of people). In other words, all queries in this work follow the form---What proportion of [groups/individuals] satisfy predicate condition $C$?---where $C$ depends on (1) the class (\textit{group} or \textit{individual}) that the query belongs and (2) the domain of the attributes ($\gG$ or $\gI$) that $C$ specifies over.
%
% \footnote{Note that we can convert $\gX$, which is a domain over groups, to a domain over individual types $\gY = \gI \times \gG \times \tilde{\gI}^{M-1}$. Here, $\gI$ defines the features for some individual row $x$, while $\gG$ defines the group to which $x$ belongs and $\tilde{\gI}^{M-1}$ the remaining rows belonging to the same group. Now, it is possible to represent \textit{individual}-level queries $q \in \gQ_I$ using a predicate condition on $x \in \gY$ (i.e. $\phi: \gY \rightarrow \cc{0, 1}$}

We summarize in Table \ref{tab:query_types} the various predicate conditions for both \textit{group} and \textit{individual}-level queries that we consider, using a $1$-way marginal function as the predicate for the examples provided. Given some set $S_G$ of \textit{group}-level attributes and set $S_I$ of \textit{individual}-level attributes where $k = |S_G| + |S_I|$, we construct a set of \textit{group} and \textit{individual}-level queries by combining predicate conditions $C_i$ for each attribute in $S_G \cup S_I$. In other words, each query condition is the conjunction of $k$ predicate conditions found in Table \ref{tab:query_types}. For example, given the \textit{group}-level attribute \textsc{Urban/rural} and \textit{individual}-level attributes \textsc{Sex} and \textsc{Race}, we have queries of the following form: 
%
\begin{itemize}
    \setlength\itemsep{0em}
    \item ($\gQ_G$) What proportion of \textit{households} are located in an \textbf{urban} area and contain \textit{at least one individual} who is \textbf{female} and \textbf{white}?
    \item ($\gQ_I$) What proportion of \textit{individuals} reside in a household located in an \textbf{urban} area and are \textbf{female} and \textbf{white}? 
\end{itemize}

\input{tables/query_types}

\textbf{Sensitivity of $\gQ$.} Typical private query release settings operate under a definition of \textit{bounded} differential privacy, where \textit{neighboring datasets} $D, D'$ are to defined to be such that $N = |D| = |D'|$ is given (perhaps under the assumption that it is public knowledge). In this setting, we have a dataset $D \in \gX$ with $N_I$ individual rows comprising $N_G$ groups. Therefore, we similarly assume for that both $N_G$ and $N_I$ are given (and fixed). For example, for release of census survey data, the U.S. Census Bureau may publish both the total number of people in the United States, as well as, the total number of households that such people reside in. Furthermore, we assume that while $D$ and $D'$ still differ on an individual row, the total number of groups and maximum group size $M$ remain the same. Under this assumption then, we have that $\gQ_G$ and $\gQ_I$ are comprised of \linears normalized by constants $N = N_G$ and $N = N_I$ respectively. Therefore, we also have that the $\ell_1$-sensitivities of queries in $\gQ_G$ and $\gQ_I$ are $\frac{1}{N_G}$ and $\frac{1}{N_I}$ respectively.






% \footnote{We note that there exists a non-exhaustive list of ways in which one can measure the composition of individual rows within a group (Table \ref{tab:query_types}, $2^{nd}$ row: \textit{group}-level queries where $\textrm{Domain}(\phi) = \gI$). For example, instead of asking whether a household has \textit{at least one} male, one can instead ask if \textit{at least half} of individuals are male of whether the household is entirely male. Alternatively, one can query for more exact counts, such as whether the household \textit{has exactly} $3$ males.}

%%%%%%%%%%%%%%%%%%%%%%
\iffalse
Using our representation of the data domain $\gX$, we can then write a \textit{group}-level hierarchical query as a \normcounting that is defined only by a single predicate condition. However, because a single group in $\gX$ may contribute up to $M$ individual rows to the total count (i.e., $\phi: \gX \rightarrow \cc{0, 1, \ldots, M}$), we cannot write \textit{individual}-level queries in the same way using $\gX$. Therefore, we introduce the corresponding data domain 
%
\begin{equation*}
    \gY = \gI \times \gG \times \tilde{\gI}^{M-1}
\end{equation*}
%
that represents hierarchical data at the $\textit{individual}-level$ with $\gI$ defining the features for some individual row $x$, $\gG$ the group to which $x$ belongs, and $\tilde{\gI}^{M-1}$ the remaining rows belonging to the same group. In this simple way, we can convert any hierarchical dataset from a collection of groups to a collection of individuals contained in such groups. Now, it is possible to represent each $\textit{individual}-level$ query $q \in \gQ_I$ as a \normcounting using some predicate condition as well (as we later do in in our method \hpd).
%  We will show later in Section \ref{sec:modeling} that it is useful to define \textit{individual}-level queries as \normcountings so that they too can be specified by a single indicator function $\phi$.
\fi
%%%%%%%%%%%%%%%%%%%%%%

==> notes/old3/model.tex <==
\subsection{old stuff}

In the non-hierarchical setting (i.e. data are only at the \textit{individual-level}), \citet{liu2021iterative} demonstrate that one can represent any data domain $\gI$ as product distributions over each attribute in $\gI$, which we denote as $P_{\gI}$. However, in the hierarchical setting, there exists attributes at the \textit{group-level}, requiring us to model a separate distribution $P_{\gG}$ over $\gG$ as well. Moreover, given that each household has at most $M$ individuals, we propose maintaining a separate distribution $P_{\gI_{i}}$ for $i \in \cc{1, 2, \ldots, M}$, where each $P_{\gI_{i}}$ corresponds to the $i^{th}$ possible person in a household. Finally, because the size of a group can vary (i.e., $\tilde{\gI}$ may be a non-existent individual row $\perp$), we let $P_{\textrm{\#}}$ be a discrete distribution over possible group sizes $m$. We let $P$ denote the overall distribution over $\gX$  given by $P_{\textrm{\#}}$, $P_{\gG}$, and $P_{\gI_{i}}$ for $i \in \cc{1, 2, \ldots, M}$.

\textit{Mixture of product distributions.}
%
Modeling any dataset $D$ using $P_{\textrm{\#}}$, $P_{\gG}$, and $P_{\gI_{i}}$ assumes that for all groups and the individual rows contained each group, attributes are independent. Therefore, we maintain a set of $K$ product distributions $P^{(k)}$ for $k \in \cc{1, 2, \ldots, K}$, where $K$ is some tunable parameter that increases the expressiveness of our probability distribution $P$.
%
\footnote{For example, dataset $D$ of size $N$ can be perfectly captured by a set of $K = N$ product distributions (i.e., a product distribution of point masses for each row in $D$).}
%
Going forward, we let $P = \cc{P^{(1)}, P^{(2)}, \ldots, P^{(K)}}$, meaning that $P$ is parameterized by $d' = K \times (M + |\gG| + M |\gI|)$ values. To sample from $P$, we first sample uniformly some $P^{(k)}$ from the set of $K$ distributions and then follow the sampling procedure summarized in Algorithm \ref{alg:hpd_sampling}.

% \textit{Sampling.} 
% %
% To sample rows from $P_{\textrm{hier}}$, we propose a simple $2$-stage sampling procedure. First, we sample from $P_{\gG}$ a set of attributes in $\gG$ to define the group-level features, as well as the number of individual rows $m$ in each group from $P_{\textrm{\#}}$. Subsequently, we sample $m$ sets of individual-level attributes $\gI$ according to the distributions $P_{\gI_{1}}, P_{\gI_{2}}, \ldots, P_{\gI_{M}}$. Note that we will sample groups uniformly from each $P_{\textrm{hier}}^{(k)}$ (e.g., if $K=10$ and we wish to sample $500$ rows for our synthetic dataset, we sample $50$ groups from each distribution $P_{\textrm{hier}}^{(k)}$).
% (i.e. in a group of size $m$, $P_{\gI_{1}}, P_{\gI_{2}}, \ldots, P_{\gI_{M}}$ are designated as the distributions from which individual row's attributes are drawn from)

\subsubsection{Modeling}

We now show how one can derive iterative algorithms for hierarchical data under the \adaptive framework \citep{liu2021iterative}. In particular, having restricted our family of distributions $\gD$ over $X$ to the set of product distributions $P_{\textrm{hier}}$, we simply need to (1) parametrize $P_{\textrm{hier}}$ and (2) derive a loss function that is differentiable w.r.t to such parameters.

\textit{Parametrizing $P_{\textrm{hier}}$.} 
%
In this setting, any algorithm must output some $d'$-dimensional vector that is made up of the probability vectors in $P_{\textrm{hier}}$. For notational purposes, we will let $\vect{P}^{\gG}$ be a $(K \times |\gG|)$-dimensional matrix where each row vector $\vect{P}^{\gG}_k$ corresponds to \textit{group-level} distribution $P_{\gG}^{(k)}$. Similarly, let $\vect{P}^{\gI_{i}}$ be a $(K \times |\gI|)$-dimensional matrix corresponding to $P_{\gI_{i}}$ for each $i \in \cc{1, 2, \ldots, M}$ and $\vect{P}^{\textrm{\#}}$ be a $(K \times M)$-dimensional matrix corresponding to $P_{\textrm{\#}}$.
%
% \footnote{Note that since we have a separate matrix parameterizing $\gG$, $\gI_i$ and $M$, it is simple to switch between viewing $P_\textrm{hier}$ as a distribution over either \textit{groups} ($\gG$) or \textit{individuals} ($\gI$). Similarly, calculating \normcountings at the \textit{group-level} and \textit{individual-level} is equivalent to looping over each row in $\vect{P}^{\gG}$ and $\vect{P}^{\gI_{i}}$ respectively.}

We describe two methods for parameterizing $P_{\textrm{hier}}$ that are inspired by \rapsoftmax and \gem \citep{liu2021iterative}. The first of which maintains a fixed distribution in which the parameters of our model are exactly the probabilities vectors that comprise $P_{\textrm{hier}}$, and the second of which employs generative modeling by employing some neural network architecture that takes as input randomly sampled Gaussian noise $\vect{z}$. Note that in both cases, we use the softmax function over dimensions corresponding to each attribute to output probabilty matrices $\vect{P}^{\gG}$, $\vect{P}^{\gI_{i}}$, and $\vect{P}^{\textrm{\#}}$. 

\textbf{Fixed distribution modeling (\fixed).} 
%
Our first method defines a "model" whose parameters $\theta^{\gG}$, $\theta^{\gI_{i}}$, and $\theta^{\textrm{\#}}$ are simply the  matrices $\vect{P}^{\gG}$, $\vect{P}^{\gI_{i}}$, and $\vect{P}^{\textrm{\#}}$ respectively.

\textbf{Generative modeling (\generative).} 
%
Alternatively, we propose using a a multi-headed neural network $F$ to generate rows from Gaussian noise $\rvz \sim \gN(0, I_{K})$. In this case, the output of each head, which we denote by $F^{\gG}(\rvz)$, $F^{\gI_{i}}(\rvz)$, and $F^{\textrm{\#}}(\rvz)$, corresponds to the $\vect{P}^{\gG}$, $\vect{P}^{\gI_{i}}$, and $\vect{P}^{\textrm{\#}}$ respectively.

% For our experiments, we use an MLP (with residual connections) for $F$, where $F_G$ is the concatenation of $M$ separate product distributions that we designate as $F_{I,1} \ldots F_{I,M}$. 

% We present two methods optimizing $P_{\textrm{hier}}$ over some set of hierarchical queries $\gQ$, the former being inspired by \rapsoftmax

\textit{Loss function.}
%
Following the \adaptive framework \citep{liu2021iterative}, at each round $t$, we have a set of selected queries $\tilde{Q}_{1:t} = \cc{\tilde{q}_1, \ldots, \tilde{q}_t}$ and their noisy measurements $\tilde{M}_{1:t} = \cc{\tilde{m}_1, \ldots, \tilde{m}_t}$. Suppose we have some set of probability matrices $\vect{P}^{\gG}$, $\vect{P}^{\gI_{i}}$ for $i \in \cc{1, 2, \ldots, M}$, and $\vect{P}^{\textrm{\#}}$ that are generated via either the fixed distribution or generative modeling methods outlined above. Abusing notation, we use $\vect{P}$ to denote the collection of these matrices. Then at each round $t$, we optimize the following differentiable loss function via stochastic gradient descent:
%
\begin{equation}\label{eq:hpd_loss}
    \gL^{\hpd} \pp{\vect{P}, \tilde{Q}_{1:t}, \tilde{M}_{1:t}} = 
    \sum_{i=1}^{t} \norm{\tilde{m}_i - f_{\tilde{q}_i} \pp{\vect{P}} }_2
\end{equation}
%
where for query $q$, there exists a corresponding function $f_q$ that maps from $\vect{P}^{\gG}$, $\vect{P}^{\gI_{i}}$ for $i \in \cc{1, 2, \ldots, M}$, and $\vect{P}^{\textrm{\#}}$ to the corresponding query answer. Referring to the query types in Table \ref{tab:query_types}, we have that 
%
\begin{equation*}
    f_{q} \pp{\vect{P}} = 
    \frac{1}{K} \sum_{k=1}^K \pp{\prod_{i \in S_G} \vect{P}^{\gG}_{ki}} 
    \pp{\sum_{m=1}^{M} \vect{P}^{\textrm{\#}}_{km} \pp{1 - \prod_{j=1}^{m}{\pp{1 - \prod_{i \in S_I} \vect{P}^{\gI_{j}}_{ki} }}}}
\end{equation*}
%
for \textit{group}-level hierarchical queries ($\gQ_G$) and
%    

\begin{equation*}
    \left.
    f_{q} \pp{\vect{P}} = 
    \frac{1}{K} \sum_{k=1}^K 
    \pp{\prod_{i \in S_G} \vect{P}^{\gG}_{ki}} 
    \pp{\sum_{m=1}^M \vect{P}^{\textrm{\#}}_{km} \sum_{j=1}^{m} \pp{\prod_{i \in S_I} \vect{P}^{\gI_{j}}_{ki} }}
    \middle/
    \sum_{k=1}^K 
    \pp{\sum_{m=1}^M m \vect{P}^{\textrm{\#}}_{km}}
    \right.
\end{equation*}   
%
for \textit{individual}-level hierarchical queries ($\gQ_I$). \swcomment{should mention that the $f_q$ above are differentiable}
% \begin{equation*}
% \begin{gathered}
%     f_{q} \pp{\vect{P}} = 
%     \frac{f_{q, 1} 
%     \pp{\vect{P}}}{f_{q, 2} \pp{\vect{P}}} \\
%     f_{q, 1} \pp{\vect{P}} = 
%     \sum_{k=1}^K \sum_{m=1}^M \vect{P}^{\textrm{\#}}_{km} \pp{\sum_{j=1}^{m} \pp{\prod_{i \in S_I} \vect{P}^{\gI_{j}}_{ki} }}
%     \pp{\prod_{i \in S_G} \vect{P}^{\gG}_{ki}} \\
%     f_{q, 2} \pp{\vect{P}} = \sum_{k=1}^K \sum_{m=1}^M m \vect{P}^{\textrm{\#}}_{km}
% \end{gathered}
% \end{equation*} 

\iffalse



\subsection{Explicit distribution over the support of $\gX$}

First, we consider algorithms that optimize over the distributional family $\gD = \cc{\rvx \mid \rvx \in [0, 1]^d, \norm{\rvx}_1 = 1}$. In other words, $\gD$ contains all possible probability distributions over $\gX$, and any histogram $A \in \gD$ can be thought of as a normalized histogram over group types in $\gX$. In this case, the parameters of methods optimizing over such representations are simply the values of a $|\gX|$-dimensional probability vector. Furthermore, we can also sample directly from $A_D$ to generate a synthetic dataset $\hat{D} \in \gX$.

Suppose we have some dataset $D \in \gX$ with some group size $N_G$ and histogram representation $A_D \in \gD$. Then, we can write any \linear (Definition \ref{def:linear_query}) as a dot product $q_{\phi}(D) = N_G \langle \vec{q}_\phi, A_D \rangle$ and $\vec{q}_\phi = \lbrack \phi(\rvx_1), \ldots, \phi(\rvx_d) \rbrack$. We now discuss how to evaluate both \textit{group} and \textit{individual-level} queries on a histogram $A \in \gD$.

\textit{Group-level queries} ($\gQ_G$).
%
Given that $A$ is a distribution over all possible group types, we have that $\phi:\gX \rightarrow \cc{0, 1}$. Moreover, since we are normalizing over some total number of groups $N_G$ for \textit{group}-level queries, our query function $f_q$ for some query with predicate $\phi$ is simply
%
\begin{align*}
    f_{q}(A) = \frac{1}{N_G} q_{\phi}(A) = \langle \vec{q}_\phi, A \rangle
\end{align*}

\textit{Individual-level queries} ($\gQ_I$).
%
A group can contribute up to $M$ individuals when counting the number of individuals satisfying some predicate condition $\phi:\gX \rightarrow \cc{0, 1, \ldots, M}$. Moreover, even when $N_G$ is fixed, the number of individual rows contained in $D$ varies with $A_D$. Let $\phi_{\#}:\gX \rightarrow \cc{1, 2, \ldots, M}$ be the predicate function that outputs the size of a group $x \in \gX$. Then the total number of individual rows in $D$ is $N_I = N_G \langle \vec{q}_{\phi_{\#}}, A_D \rangle$. Therefore for \textit{individual}-level queries, we have that
%
\begin{align*}
    f_{q}(A) = \frac{1}{N_I} q_{\phi}(A) = \frac{ \langle \vec{q}_{\phi}, A \rangle}{\langle \vec{q}_{\phi_{\#}}, A \rangle}
\end{align*}

Having described how to both parameterize $\gX$ and evaluate any hierarchical query $q$ on some dataset $D \in \gX$, one can directly optimize our objective using algorithms such as the \textit{multiplicative weights} update rule (i.e., the \mwem algorithm \citep{HardtLM12}, which we describe in Appendix \ref{appx:mwem}). 

\fi
